Revisiting neutron starquakes caused by spin-down

Pulsars show a steady decrease in their rotational frequency, occasionally interrupted by sudden spin-ups called glitches, whose physical origin is still a mystery. One suggested explanation for at least the small glitches are starquakes, that is, failures of the solid neutron star crust, in which the progressive reduction in the centrifugal force deforms the star, stressing the solid until it breaks. This produces a spin-up, dissipating energy inside the star. We analyze the deformations produced by the decreasing centrifugal force, modeling the star with a fluid core and a solid crust, each with uniform density and with the core possibly denser than the crust, as a simple approximation to the strong density gradient present in real neutron stars. The deformation is qualitatively different from the previously studied case of equal densities. The former more closely resembles the behavior of a fluid star, in which the core-crust interface is a surface of constant gravitational plus centrifugal potential. Regardless of the uncertain breaking strain, the glitch activity in this model is several orders of magnitude smaller than observed, even if only small glitches are considered. For a large breaking strain, suggested by simulations, glitches due to starquakes could be roughly of the correct size but much less frequent than observed glitches. The energy released in each glitch is much larger than in the model of angular momentum transfer from a faster rotating superfluid in the inner crust. On the other hand, we cannot rule out that the heating produced by small starquakes could trigger glitches by allowing neutron superfluid vortices to move. We also confirm that stresses in the neutron star crust can in principle support an ellipticity much larger than some observational upper limits from pulsar timing and continuous gravitational wave searches.

==> 1starticle1.tex <==

@book{love1920treatise,
  title={A treatise on the mathematical theory of elasticity},
  author={Love, Augustus Edward Hough},
  year={1920},
  publisher={at the University Press}
}

@ARTICLE{1968Natur.217..709H,
       author = {{Hewish}, A. and {Bell}, S.~J. and {Pilkington}, J.~D.~H. and {Scott},
        P.~F. and {Collins}, R.~A.},
        title = "{Observation of a Rapidly Pulsating Radio Source}",
      journal = {\nat},
         year = 1968,
        month = Feb,
       volume = {217},
        pages = {709-713},
          doi = {10.1038/217709a0},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1968Natur.217..709H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969Natur.222..228R,
       author = {{Radhakrishnan}, V. and {Manchester}, R.~N.},
        title = "{Detection of a Change of State in the Pulsar PSR 0833-45}",
      journal = {\nat},
         year = 1969,
        month = Apr,
       volume = {222},
        pages = {228-229},
          doi = {10.1038/222228a0},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1969Natur.222..228R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969IAUC.2179....1B,
       author = {{Boynton}, P.~E. and {Groth}, E.~J., III and {Partridge}, R.~B. and
        {Wilkinson}, D.~T.},
        title = "{Apparent change in frequency of NP 0532.}",
      journal = {International Astronomical Union Circular},
         year = 1969,
        month = Jan,
       volume = {2179},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/1969IAUC.2179....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1969Natur.223..597R,
   author = {{Ruderman}, M.},
    title = "{Neutron Starquakes and Pulsar Periods}",
  journal = {\nat},
     year = 1969,
    month = aug,
   volume = 223,
    pages = {597-598},
      doi = {10.1038/223597b0},
   adsurl = {http://adsabs.harvard.edu/abs/1969Natur.223..597R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969Natur.224..872B,
   author = {{Baym}, G. and {Pethick}, C. and {Pines}, D. and {Ruderman}, M.
	},
    title = "{Spin Up in Neutron Stars : The Future of the Vela Pulsar}",
  journal = {\nat},
     year = 1969,
    month = nov,
   volume = 224,
    pages = {872-874},
      doi = {10.1038/224872a0},
   adsurl = {http://adsabs.harvard.edu/abs/1969Natur.224..872B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1971AnPhy..66..816B,
   author = {{Baym}, G. and {Pines}, D.},
    title = "{Neutron starquakes and pulsar speedup.}",
  journal = {Annals of Physics},
     year = 1971,
   volume = 66,
    pages = {816-835},
      doi = {10.1016/0003-4916(71)90084-4},
   adsurl = {http://adsabs.harvard.edu/abs/1971AnPhy..66..816B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1975Natur.256...25A,
   author = {{Anderson}, P.~W. and {Itoh}, N.},
    title = "{Pulsar glitches and restlessness as a hard superfluidity phenomenon}",
  journal = {\nat},
 keywords = {Neutron Stars, Pulsars, Stellar Structure, Superfluidity, Vorticity, Astronomical Models, Proton Flux Density, Stellar Magnetic Fields, Superconductivity},
     year = 1975,
    month = jul,
   volume = 256,
    pages = {25-27},
      doi = {10.1038/256025a0},
   adsurl = {http://adsabs.harvard.edu/abs/1975Natur.256...25A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1976ApJ...203..213R,
       author = {{Ruderman}, M.},
        title = "{Crust-breaking by neutron superfluids and the Vela pulsar glitches.}",
      journal = {\apj},
     keywords = {Neutron Stars, Pulsars, Spin Dynamics, Stellar Rotation, Superfluidity, Angular Momentum, Angular Velocity, Momentum Transfer, Astrophysics},
         year = 1976,
        month = Jan,
       volume = {203},
        pages = {213-222},
          doi = {10.1086/154069},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1976ApJ...203..213R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1983bhwd.book.....S,
       author = {{Shapiro}, Stuart L. and {Teukolsky}, Saul A.},
        title = "{Black holes, white dwarfs, and neutron stars : the physics of compact objects}",
         year = "1983",
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983bhwd.book.....S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1988ApJ...325..725M,
   author = {{McDermott}, P.~N. and {van Horn}, H.~M. and {Hansen}, C.~J.
	},
    title = "{Nonradial oscillations of neutron stars}",
  journal = {\apj},
 keywords = {Neutron Stars, Pulsars, Stellar Models, Stellar Oscillations, Elastic Waves, Stellar Gravitation, Stellar Interiors, Stellar Radiation, Stellar Temperature},
     year = 1988,
    month = feb,
   volume = 325,
    pages = {725-748},
      doi = {10.1086/166044},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...325..725M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1994ApJ...427L..29A,
       author = {{Alpar}, M.~A. and {Chau}, H.~F. and {Cheng}, K.~S. and {Pines}, D.},
        title = "{Postglitch Relaxation of the Crab Pulsar: Evidence for Crust Cracking}",
      journal = {\apj},
     keywords = {Astrophysics, Crab Nebula, Cracking (Fracturing), Crusts, Neutron Stars, Pulsars, Relaxation (Mechanics), Starquakes, Stellar Models, Angular Acceleration, Angular Momentum, Angular Velocity, Variations, Astrophysics, DENSE MATTER, STARS: PULSARS: INDIVIDUAL NAME: CRAB PULSAR, STARS: NEUTRON},
         year = 1994,
        month = May,
       volume = {427},
        pages = {L29},
          doi = {10.1086/187357},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1994ApJ...427L..29A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1999PhRvL..83.3362L,
   author = {{Link}, B. and {Epstein}, R.~I. and {Lattimer}, J.~M.},
    title = "{Pulsar Constraints on Neutron Star Structure and Equation of State}",
  journal = {Physical Review Letters},
   eprint = {astro-ph/9909146},
     year = 1999,
    month = oct,
   volume = 83,
    pages = {3362-3365},
      doi = {10.1103/PhysRevLett.83.3362},
   adsurl = {http://adsabs.harvard.edu/abs/1999PhRvL..83.3362L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000MNRAS.319..902U,
       author = {{Ushomirsky}, Greg and {Cutler}, Curt and {Bildsten}, Lars},
        title = "{Deformations of accreting neutron star crusts and gravitational wave emission}",
      journal = {\mnras},
     keywords = {ACCRETION, ACCRETION DISCS, DENSE MATTER, RADIATION MECHANISMS: NON-THERMAL, STARS: NEUTRON, STARS: ROTATION, Astrophysics, General Relativity and Quantum Cosmology},
         year = 2000,
        month = Dec,
       volume = {319},
        pages = {902-932},
          doi = {10.1046/j.1365-8711.2000.03938.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0001136},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2000MNRAS.319..902U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2000ApJ...543..987F,
   author = {{Franco}, L.~M. and {Link}, B. and {Epstein}, R.~I.},
    title = "{Quaking Neutron Stars}",
  journal = {\apj},
   eprint = {astro-ph/9911105},
 keywords = {Dense Matter, Magnetic Fields, pulsars: individual (Crab pulsar), Stars: Magnetic Fields, Stars: Neutron},
     year = 2000,
    month = nov,
   volume = 543,
    pages = {987-994},
      doi = {10.1086/317121},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...543..987F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.324..811J,
       author = {{Jones}, D.~I. and {Andersson}, N.},
        title = "{Freely precessing neutron stars: model and observations}",
      journal = {\mnras},
     keywords = {STELLAR DYNAMICS, METHODS: ANALYTICAL, STARS: NEUTRON, PULSARS: GENERAL, STARS: ROTATION, Astrophysics},
         year = 2001,
        month = Jul,
       volume = {324},
        pages = {811-824},
          doi = {10.1046/j.1365-8711.2001.04251.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0011063},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2001MNRAS.324..811J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...380..151D,
       author = {{Douchin}, F. and {Haensel}, P.},
        title = "{A unified equation of state of dense matter and neutron star structure}",
      journal = {\aap},
     keywords = {DENSE MATTER, EQUATION OF STATE, STARS: NEUTRON, Astrophysics},
         year = "2001",
        month = "Dec",
       volume = {380},
        pages = {151-167},
          doi = {10.1051/0004-6361:20011402},
archivePrefix = {arXiv},
       eprint = {astro-ph/0111092},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...380..151D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2003ApJ...588..975C,
   author = {{Cutler}, C. and {Ushomirsky}, G. and {Link}, B.},
    title = "{The Crustal Rigidity of a Neutron Star and Implications for PSR B1828-11 and Other Precession Candidates}",
  journal = {\apj},
   eprint = {astro-ph/0210175},
 keywords = {Dense Matter, pulsars: individual (PSR 1828-11), Stars: Neutron, Stars: Rotation},
     year = 2003,
    month = may,
   volume = 588,
    pages = {975-991},
      doi = {10.1086/368308},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588..975C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2011MNRAS.414.1679E,
   author = {{Espinoza}, C.~M. and {Lyne}, A.~G. and {Stappers}, B.~W. and 
	{Kramer}, M.},
    title = "{A study of 315 glitches in the rotation of 102 pulsars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.1743},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, pulsars: general},
     year = 2011,
    month = jun,
   volume = 414,
    pages = {1679-1704},
      doi = {10.1111/j.1365-2966.2011.18503.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.1679E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@book{thorne2017modern,
  title={Modern Classical Physics: Optics, Fluids, Plasmas, Elasticity, Relativity, and Statistical Physics},
  author={Thorne, K.S. and Blandford, R.D.},
  isbn={9781400848898},
  url={https://books.google.cl/books?id=U1S6BQAAQBAJ},
  year={2017},
  publisher={Princeton University Press}
}

@ARTICLE{2009PhRvL.102s1102H,
   author = {{Horowitz}, C.~J. and {Kadau}, K.},
    title = "{Breaking Strain of Neutron Star Crust and Gravitational Waves}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {0904.1986},
 primaryClass = "astro-ph.SR",
 keywords = {Neutron stars, Deformation and plasticity, Structural failure of materials, Gravitational radiation detectors, mass spectrometers, and other instrumentation and techniques},
     year = 2009,
    month = may,
   volume = 102,
   number = 19,
      eid = {191102},
    pages = {191102},
      doi = {10.1103/PhysRevLett.102.191102},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhRvL.102s1102H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{sokolnikoff1956mathematical,
  title={Mathematical theory of elasticity},
  author={Sokolnikoff, Ivan Stephen and Specht, Robert Dickerson and others},
  volume={83},
  year={1956},
  publisher={McGraw-Hill New York}
}

@book{karato2012deformation,
  title={Deformation of earth materials: an introduction to the rheology of solid earth},
  author={Karato, Shun-ichiro},
  year={2012},
  publisher={Cambridge University Press}
}

@ARTICLE{2015IJMPD..2430008H,
   author = {{Haskell}, B. and {Melatos}, A.},
    title = "{Models of pulsar glitches}",
  journal = {International Journal of Modern Physics D},
archivePrefix = "arXiv",
   eprint = {1502.07062},
 primaryClass = "astro-ph.SR",
 keywords = {Pulsars, neutron stars, superfluidity, hydrodynamic aspects of, Neutron stars},
     year = 2015,
    month = jan,
   volume = 24,
      eid = {1530008},
    pages = {1530008},
      doi = {10.1142/S0218271815300086},
   adsurl = {http://adsabs.harvard.edu/abs/2015IJMPD..2430008H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.460.1201H,
   author = {{Howitt}, G. and {Haskell}, B. and {Melatos}, A.},
    title = "{Hydrodynamic simulations of pulsar glitch recovery}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1512.07903},
 primaryClass = "astro-ph.HE",
 keywords = {dense matter, hydrodynamics, stars: neutron, pulsars: general},
     year = 2016,
    month = aug,
   volume = 460,
    pages = {1201-1213},
      doi = {10.1093/mnras/stw1043},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460.1201H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...743L..20P,
   author = {{Pizzochero}, P.~M.},
    title = "{Angular Momentum Transfer in Vela-like Pulsar Glitches}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1105.0156},
 primaryClass = "astro-ph.HE",
 keywords = {dense matter, pulsars: general, pulsars: individual: PSR J0835-4510, stars: neutron},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {L20},
    pages = {L20},
      doi = {10.1088/2041-8205/743/1/L20},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743L..20P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.449.3559H,
   author = {{Hooker}, J. and {Newton}, W.~G. and {Li}, B.-A.},
    title = "{Efficacy of crustal superfluid neutrons in pulsar glitch models}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.0031},
 primaryClass = "astro-ph.SR",
 keywords = {dense matter, equation of state, stars: neutron, pulsars: general, pulsars: individual: Vela},
     year = 2015,
    month = jun,
   volume = 449,
    pages = {3559-3567},
      doi = {10.1093/mnras/stv582},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.3559H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016MNRAS.461.2809M,
   author = {{McKee}, J.~W. and {Janssen}, G.~H. and {Stappers}, B.~W. and 
	{Lyne}, A.~G. and {Caballero}, R.~N. and {Lentati}, L. and {Desvignes}, G. and 
	{Jessner}, A. and {Jordan}, C.~A. and {Karuppusamy}, R. and 
	{Kramer}, M. and {Cognard}, I. and {Champion}, D.~J. and {Graikou}, E. and 
	{Lazarus}, P. and {Os{\l}owski}, S. and {Perrodin}, D. and {Shaifullah}, G. and 
	{Tiburzi}, C. and {Verbiest}, J.~P.~W.},
    title = "{A glitch in the millisecond pulsar J0613-0200}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1606.04098},
 primaryClass = "astro-ph.HE",
     year = 2016,
    month = sep,
   volume = 461,
    pages = {2809-2817},
      doi = {10.1093/mnras/stw1442},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461.2809M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000MNRAS.315..534L,
   author = {{Lyne}, A.~G. and {Shemar}, S.~L. and {Smith}, F.~G.},
    title = "{Statistical studies of pulsar glitches}",
  journal = {\mnras},
 keywords = {PULSARS: GENERAL, PULSARS: INDIVIDUAL: VELA, PULSARS: INDIVIDUAL: CRAB},
     year = 2000,
    month = jul,
   volume = 315,
    pages = {534-542},
      doi = {10.1046/j.1365-8711.2000.03415.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.315..534L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PROCEEDINGS{2007ASSL..326.....H,
    title = "{Neutron Stars 1 : Equation of State and Structure}",
 keywords = {NEUTRON STARS, CORES, PLASMA PHYSICS, MAGNETIC FIELDS, CRUST},
booktitle = {Astrophysics and Space Science Library},
     year = 2007,
   series = {Astrophysics and Space Science Library},
   volume = 326,
   editor = {{Haensel}, P. and {Potekhin}, A.~Y. and {Yakovlev}, D.~G.},
    pages = {Haensel},
   adsurl = {http://adsabs.harvard.edu/abs/2007ASSL..326.....H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Chamel2008,
author="Chamel, Nicolas
and Haensel, Pawel",
title="Physics of Neutron Star Crusts",
journal="Living Reviews in Relativity",
year="2008",
volume="11",
number="1",
pages="10",
abstract="The physics of neutron star crusts is vast, involving many different research fields, from nuclear and condensed matter physics to general relativity. This review summarizes the progress, which has been achieved over the last few years, in modeling neutron star crusts, both at the microscopic and macroscopic levels. The confrontation of these theoretical models with observations is also briefly discussed.",
issn="1433-8351",
doi="10.12942/lrr-2008-10",
url="http://dx.doi.org/10.12942/lrr-2008-10"
}

@ARTICLE{1970PhRvL..24..923S,
   author = {{Smoluchowski}, R.},
    title = "{Frequency of Pulsar Starquakes}",
  journal = {Physical Review Letters},
     year = 1970,
    month = apr,
   volume = 24,
    pages = {923-925},
      doi = {10.1103/PhysRevLett.24.923},
   adsurl = {http://adsabs.harvard.edu/abs/1970PhRvL..24..923S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000Natur.406..484S,
   author = {{Stairs}, I.~H. and {Lyne}, A.~G. and {Shemar}, S.~L.},
    title = "{Evidence for free precession in a pulsar}",
  journal = {\nat},
     year = 2000,
    month = aug,
   volume = 406,
    pages = {484-486},
      doi = {10.1038/35020010},
   adsurl = {http://adsabs.harvard.edu/abs/2000Natur.406..484S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012MNRAS.426.2404H,
   author = {{Hoffman}, K. and {Heyl}, J.},
    title = "{Mechanical properties of non-accreting neutron star crusts}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.3258},
 primaryClass = "astro-ph.SR",
 keywords = {dense matter, stars: magnetars, stars: neutron, pulsars: general},
     year = 2012,
    month = nov,
   volume = 426,
    pages = {2404-2412},
      doi = {10.1111/j.1365-2966.2012.21921.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.2404H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{christensen2013theory,
  title={The Theory of Materials Failure},
  author={Christensen, R.M.},
  isbn={9780191638220},
  url={https://books.google.es/books?id=7pdoAgAAQBAJ},
  year={2013},
  publisher={OUP Oxford}
}

@article{PhysRevB.80.132104,
  title = {Limits to Poisson's ratio in isotropic materials},
  author = {Mott, P. H. and Roland, C. M.},
  journal = {Phys. Rev. B},
  volume = {80},
  issue = {13},
  pages = {132104},
  numpages = {4},
  year = {2009},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.80.132104},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.80.132104}
}

@article{baiko2011,
author = {Baiko, D. A.},
title = {Shear modulus of neutron star crust},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {416},
number = {1},
pages = {22},
year = {2011},
doi = {10.1111/j.1365-2966.2011.18819.x},
URL = { + http://dx.doi.org/10.1111/j.1365-2966.2011.18819.x},
eprint = {/oup/backfile/content_public/journal/mnras/416/1/10.1111/j.1365-2966.2011.18819.x/2/mnras0416-0022.pdf}
}

@article{1742-6596-342-1-012005,
  author={Joseph Hughto},
  title={Structure and Shear Modulus of the Neutron Star Crust},
  journal={Journal of Physics: Conference Series},
  volume={342},
  number={1},
  pages={012005},
  url={http://stacks.iop.org/1742-6596/342/i=1/a=012005},
  year={2012},
  abstract={A thorough understanding of the neutron star crust is necessary to describe some observations of transient events such as quasi-periodic oscillations after magnetar giant flares and cooling following outbursts in low-mass X-ray binaries. I perform molecular dynamics simulations to model the crystalline structure of the crust and also compute shear modulus and liquid-solid phase diagrams.}
}

@ARTICLE{2006ApJ...652.1531M,
       author = {{Middleditch}, J. and {Marshall}, F.~E. and {Wang}, Q.~D. and
        {Gotthelf}, E.~V. and {Zhang}, W.},
        title = "{Predicting the Starquakes in PSR J0537-6910}",
      journal = {\apj},
     keywords = {Stars: Pulsars: Individual: Alphanumeric: PSR J0537-6910, Stars: Neutron, X-Rays: Stars, Astrophysics},
         year = 2006,
        month = Dec,
       volume = {652},
        pages = {1531-1546},
          doi = {10.1086/508736},
archivePrefix = {arXiv},
       eprint = {astro-ph/0605007},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2006ApJ...652.1531M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2008arXiv0812.2650H,
       author = {{Horowitz}, C.~J. and {Hughto}, J.},
        title = "{Molecular Dynamics Simulation of Shear Moduli for Coulomb Crystals}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics},
         year = "2008",
        month = "Dec",
          eid = {arXiv:0812.2650},
        pages = {arXiv:0812.2650},
archivePrefix = {arXiv},
       eprint = {0812.2650},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008arXiv0812.2650H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...491..489Z,
       author = {{Zdunik}, J.~L. and {Bejger}, M. and {Haensel}, P.},
        title = "{Deformation and crustal rigidity of rotating neutron stars}",
      journal = {\aap},
     keywords = {dense matter, equation of state, stars: neutron, Astrophysics},
         year = 2008,
        month = Nov,
       volume = {491},
        pages = {489-498},
          doi = {10.1051/0004-6361:200810183},
archivePrefix = {arXiv},
       eprint = {0805.1814},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2008A&A...491..489Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012MNRAS.427.1574L,
       author = {{Levin}, Yuri and {Lyutikov}, Maxim},
        title = "{On the dynamics of mechanical failures in magnetized neutron star crusts}",
      journal = {\mnras},
     keywords = {stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = Dec,
       volume = {427},
        pages = {1574-1579},
          doi = {10.1111/j.1365-2966.2012.22016.x},
archivePrefix = {arXiv},
       eprint = {1204.2605},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2012MNRAS.427.1574L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2017PhRvD..96d3002O,
       author = {{Ofengeim}, D.~D. and {Fortin}, M. and {Haensel}, P. and {Yakovlev}, D.~G. and {Zdunik}, J.~L.},
        title = "{Neutrino luminosities and heat capacities of neutron stars in analytic form}",
      journal = {\prd},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = aug,
       volume = {96},
       number = {4},
          eid = {043002},
        pages = {043002},
          doi = {10.1103/PhysRevD.96.043002},
archivePrefix = {arXiv},
       eprint = {1708.08272},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017PhRvD..96d3002O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2017A&A...608A.131F,
   author = {{Fuentes}, J.~R. and {Espinoza}, C.~M. and {Reisenegger}, A. and 
	{Shaw}, B. and {Stappers}, B.~W. and {Lyne}, A.~G.},
    title = "{The glitch activity of neutron stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1710.00952},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, stars: magnetars, pulsars: general, stars: rotation},
     year = 2017,
    month = dec,
   volume = 608,
      eid = {A131},
    pages = {A131},
      doi = {10.1051/0004-6361/201731519},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...608A.131F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2017PhRvL.118z1101J,
       author = {{Jones}, D.~I. and {Ashton}, G. and {Prix}, R.},
        title = "{Implications of the Occurrence of Glitches in Pulsar Free Precession Candidates}",
      journal = {\prl},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = Jun,
       volume = {118},
          eid = {261101},
        pages = {261101},
          doi = {10.1103/PhysRevLett.118.261101},
archivePrefix = {arXiv},
       eprint = {1610.03509},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017PhRvL.118z1101J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018MNRAS.473..621A,
   author = {{Akbal}, O. and {Alpar}, M.~A.},
    title = "{Minimum glitch of the Crab pulsar and the crustquake as a trigger mechanism}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1707.01160},
 primaryClass = "astro-ph.HE",
 keywords = {dense matter, stars: neutron, pulsars: general, pulsars: individual: Crab},
     year = 2018,
    month = jan,
   volume = 473,
    pages = {621-624},
      doi = {10.1093/mnras/stx2378},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473..621A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018arXiv180404952F,
       author = {{Fattoyev}, F.~J. and {Horowitz}, C.~J. and {Lu}, Hao},
        title = "{Crust breaking and the limiting rotational frequency of neutron stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology, Nuclear Theory},
         year = 2018,
        month = Apr,
          eid = {arXiv:1804.04952},
        pages = {arXiv:1804.04952},
archivePrefix = {arXiv},
       eprint = {1804.04952},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018arXiv180404952F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Schutz09,
   author = {{Schutz}, B.},
    title = "{A First Course in General Relativity}",
booktitle = {A First Course in General Relativity by Bernard Schutz.~Cambridge University Press, 2009.~ISBN: 9780521887052},
     year = 2009,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2009fcgr.book.....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1975AnPhy..95...74C,
   author = {{Carter}, B. and {Quintana}, H.},
    title = "{Relativistic formulation of the neutron starquake theory of pulsar glitches}",
  journal = {Annals of Physics},
     year = 1975,
    month = nov,
   volume = 95,
    pages = {74-89},
      doi = {10.1016/0003-4916(75)90044-5},
   adsurl = {http://adsabs.harvard.edu/abs/1975AnPhy..95...74C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1998ApJ...508..838L,
   author = {{Link}, B. and {Franco}, L.~M. and {Epstein}, R.~I.},
    title = "{Starquake-induced Magnetic Field and Torque Evolution in Neutron Stars}",
  journal = {\apj},
   eprint = {astro-ph/9805115},
 keywords = {DENSE MATTER, MAGNETIC FIELDS, PULSARS: INDIVIDUAL (CRAB), STARS: MAGNETIC FIELDS, STARS: NEUTRON, STARS: ROTATION, Dense Matter, Magnetic Fields, pulsars: individual (Crab), Stars: Magnetic Fields, Stars: Neutron, Stars: Rotation},
     year = 1998,
    month = dec,
   volume = 508,
    pages = {838-843},
      doi = {10.1086/306457},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...508..838L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2013PhRvD..88d4004J,
   author = {{Johnson-McDaniel}, N.~K. and {Owen}, B.~J.},
    title = "{Maximum elastic deformations of relativistic stars}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1208.5227},
 primaryClass = "astro-ph.SR",
 keywords = {Wave generation and sources, Relativistic stars: structure stability and oscillations, Neutron stars},
     year = 2013,
    month = aug,
   volume = 88,
   number = 4,
      eid = {044004},
    pages = {044004},
      doi = {10.1103/PhysRevD.88.044004},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..88d4004J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...395..240R,
   author = {{Reisenegger}, A. and {Goldreich}, P.},
    title = "{A new class of g-modes in neutron stars}",
  journal = {\apj},
 keywords = {Brunt-Vaisala Frequency, Charged Particles, Hot Stars, Neutron Stars, Stellar Oscillations, Gravitational Effects, Gravitational Waves, Stellar Cores},
     year = 1992,
    month = aug,
   volume = 395,
    pages = {240-249},
      doi = {10.1086/171645},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...395..240R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987MNRAS.227..265F,
   author = {{Finn}, L.~S.},
    title = "{G-modes in zero-temperature neutron stars}",
  journal = {\mnras},
 keywords = {Ideal Fluids, Neutron Stars, Stellar Composition, Stellar Oscillations, Stellar Temperature, Vibration Mode, Isentropic Processes, Stellar Models, Temperature Dependence},
     year = 1987,
    month = jul,
   volume = 227,
    pages = {265-293},
      doi = {10.1093/mnras/227.2.265},
   adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.227..265F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1941MNRAS.101..367C,
   author = {{Cowling}, T.~G.},
    title = "{The non-radial oscillations of polytropic stars}",
  journal = {\mnras},
     year = 1941,
   volume = 101,
    pages = {367},
      doi = {10.1093/mnras/101.8.367},
   adsurl = {http://adsabs.harvard.edu/abs/1941MNRAS.101..367C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2019MNRAS.tmp.2697G,
       author = {{Giliberti}, E. and {Cambiotti}, G. and {Antonelli}, M. and
         {Pizzochero}, P.~M.},
        title = "{Modelling strains and stresses in continuously stratified rotating neutron stars}",
      journal = {\mnras},
     keywords = {stars: neutron, pulsars: general},
         year = "2019",
        month = "Nov",
        pages = {2697},
          doi = {10.1093/mnras/stz3099},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.tmp.2697G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019arXiv190206345G,
       author = {{Giliberti}, Elia and {Antonelli}, Marco and {Cambiotti}, Gabriele and
         {Pizzochero}, Pierre},
        title = "{Incompressible analytical models for spinning-down pulsars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Feb",
          eid = {arXiv:1902.06345},
        pages = {arXiv:1902.06345},
archivePrefix = {arXiv},
       eprint = {1902.06345},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190206345G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...442..749R,
       author = {{Reisenegger}, Andreas},
        title = "{Deviations from Chemical Equilibrium Due to Spin-down as an Internal Heat Source in Neutron Stars}",
      journal = {\apj},
     keywords = {Chemical Equilibrium, Heat Sources, Neutron Stars, Nuclear Reactions, Stellar Composition, Stellar Cores, Stellar Evolution, Stellar Models, Stellar Rotation, Abundance, Equations Of State, Equilibrium Equations, Neutron Emission, Reaction Kinetics, Superfluidity, Astrophysics, DENSE MATTER, EQUATION OF STATE, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, STARS: PULSARS: GENERAL, STARS: NEUTRON, Astrophysics},
         year = "1995",
        month = "Apr",
       volume = {442},
        pages = {749},
          doi = {10.1086/175480},
archivePrefix = {arXiv},
       eprint = {astro-ph/9410035},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...442..749R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.453L..36G,
       author = {{Gusakov}, M.~E. and {Kantor}, E.~M. and {Reisenegger}, A.},
        title = "{Rotation-induced deep crustal heating of millisecond pulsars}",
      journal = {\mnras},
     keywords = {stars: interiors, stars: neutron, pulsars: individual: PSR J0437-4715, stars: rotation, ultraviolet: stars, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology, Nuclear Theory},
         year = "2015",
        month = "Oct",
       volume = {453},
       number = {1},
        pages = {L36-L40},
          doi = {10.1093/mnrasl/slv095},
archivePrefix = {arXiv},
       eprint = {1507.04586},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453L..36G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018MNRAS.480.5511B,
       author = {{Baiko}, D.~A. and {Chugunov}, A.~I.},
        title = "{Breaking properties of neutron star crust}",
      journal = {\mnras},
     keywords = {dense matter, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = nov,
       volume = {480},
       number = {4},
        pages = {5511-5516},
          doi = {10.1093/mnras/sty2259},
archivePrefix = {arXiv},
       eprint = {1808.06415},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.5511B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019PASA...36...36G,
       author = {{Giliberti}, E. and {Antonelli}, M. and {Cambiotti}, G. and
         {Pizzochero}, P.~M.},
        title = "{Incompressible analytical models for spinning-down pulsars}",
      journal = {\pasa},
     keywords = {pulsars: general, stars: neutron, stars: rotation, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Jan",
       volume = {36},
          eid = {e036},
        pages = {e036},
          doi = {10.1017/pasa.2019.28},
archivePrefix = {arXiv},
       eprint = {1902.06345},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASA...36...36G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020MNRAS.491.1064G,
       author = {{Giliberti}, E. and {Cambiotti}, G. and {Antonelli}, M. and {Pizzochero}, P.~M.},
        title = "{Modelling strains and stresses in continuously stratified rotating neutron stars}",
      journal = {\mnras},
     keywords = {stars: neutron, pulsars: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jan,
       volume = {491},
       number = {1},
        pages = {1064-1078},
          doi = {10.1093/mnras/stz3099},
archivePrefix = {arXiv},
       eprint = {1809.08542},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.1064G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1983PhRvL..50.2066R,
       author = {{Ravenhall}, D.~G. and {Pethick}, C.~J. and {Wilson}, J.~R.},
        title = "{Structure of Matter below Nuclear Saturation Density}",
      journal = {\prl},
     keywords = {21.65.+f, 05.70.Fh, 97.60.-s, Nuclear matter, Phase transitions: general studies, Late stages of stellar evolution},
         year = 1983,
        month = jun,
       volume = {50},
       number = {26},
        pages = {2066-2069},
          doi = {10.1103/PhysRevLett.50.2066},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983PhRvL..50.2066R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998PhRvD..58f3001J,
       author = {{Jaranowski}, Piotr and {Kr{\'o}lak}, Andrzej and {Schutz}, Bernard F.},
        title = "{Data analysis of gravitational-wave signals from spinning neutron stars: The signal and its detection}",
      journal = {\prd},
     keywords = {95.55.Ym, 04.80.Nn, 95.75.Pq, 97.60.Gb, Gravitational radiation detectors, mass spectrometers, and other instrumentation and techniques, Gravitational wave detectors and experiments, Mathematical procedures and computer techniques, Pulsars, General Relativity and Quantum Cosmology},
         year = 1998,
        month = sep,
       volume = {58},
       number = {6},
          eid = {063001},
        pages = {063001},
          doi = {10.1103/PhysRevD.58.063001},
archivePrefix = {arXiv},
       eprint = {gr-qc/9804014},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998PhRvD..58f3001J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.500.5570G,
       author = {{Gittins}, F. and {Andersson}, N. and {Jones}, D.~I.},
        title = "{Modelling neutron star mountains}",
      journal = {\mnras},
     keywords = {gravitational waves, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics, General Relativity and Quantum Cosmology},
         year = 2021,
        month = jan,
       volume = {500},
       number = {4},
        pages = {5570-5582},
          doi = {10.1093/mnras/staa3635},
archivePrefix = {arXiv},
       eprint = {2009.12794},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.5570G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...902L..21A,
       author = {{Abbott}, R. and {Abbott}, T.~D. and {Abraham}, S. and {Acernese}, F. and {Ackley}, K. and {Adams}, A. and {Adams}, C. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Allen}, G. and {Allocca}, A. and {Altin}, P.~A. and {Amato}, A. and {Anand}, S. and {Ananyeva}, A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Angelova}, S.~V. and {Ansoldi}, S. and {Antelis}, J.~M. and {Antier}, S. and {Appert}, S. and {Arai}, K. and {Araya}, M.~C. and {Areeda}, J.~S. and {Ar{\`e}ne}, M. and {Arnaud}, N. and {Aronson}, S.~M. and {Arun}, K.~G. and {Asali}, Y. and {Ascenzi}, S. and {Ashton}, G. and {Aston}, S.~M. and {Astone}, P. and {Aubin}, F. and {Aufmuth}, P. and {AultONeal}, K. and {Austin}, C. and {Avendano}, V. and {Babak}, S. and {Badaracco}, F. and {Bader}, M.~K.~M. and {Bae}, S. and {Baer}, A.~M. and {Bagnasco}, S. and {Bailes}, M. and {Baird}, J. and {Ball}, M. and {Ballardin}, G. and {Ballmer}, S.~W. and {Bals}, A. and {Balsamo}, A. and {Baltus}, G. and {Banagiri}, S. and {Bankar}, D. and {Bankar}, R.~S. and {Barayoga}, J.~C. and {Barbieri}, C. and {Barish}, B.~C. and {Barker}, D. and {Barneo}, P. and {Barnum}, S. and {Barone}, F. and {Barr}, B. and {Barsotti}, L. and {Barsuglia}, M. and {Barta}, D. and {Bartlett}, J. and {Bartos}, I. and {Bassiri}, R. and {Basti}, A. and {Bawaj}, M. and {Bayley}, J.~C. and {Bazzan}, M. and {Becher}, B.~R. and {B{\'e}csy}, B. and {Bedakihale}, V.~M. and {Bejger}, M. and {Belahcene}, I. and {Beniwal}, D. and {Benjamin}, M.~G. and {Bennett}, T.~F. and {Bentley}, J.~D. and {Bergamin}, F. and {Berger}, B.~K. and {Bergmann}, G. and {Bernuzzi}, S. and {Bersanetti}, D. and {Bertolini}, A. and {Betzwieser}, J. and {Bhandare}, R. and {Bhandari}, A.~V. and {Bhattacharjee}, D. and {Bidler}, J. and {Bilenko}, I.~A. and {Billingsley}, G. and {Birney}, R. and {Birnholtz}, O. and {Biscans}, S. and {Bischi}, M. and {Biscoveanu}, S. and {Bisht}, A. and {Bitossi}, M. and {Bizouard}, M. -A. and {Blackburn}, J.~K. and {Blackman}, J. and {Blair}, C.~D. and {Blair}, D.~G. and {Blair}, R.~M. and {Blanch}, O. and {Bobba}, F. and {Bode}, N. and {Boer}, M. and {Boetzel}, Y. and {Bogaert}, G. and {Boldrini}, M. and {Bondu}, F. and {Bonnand}, R. and {Booker}, P. and {Boom}, B.~A. and {Bork}, R. and {Boschi}, V. and {Bose}, S. and {Bossilkov}, V. and {Boudart}, V. and {Bouffanais}, Y. and {Bozzi}, A. and {Bradaschia}, C. and {Brady}, P.~R. and {Bramley}, A. and {Branchesi}, M. and {Brau}, J.~E. and {Breschi}, M. and {Briant}, T. and {Briggs}, J.~H. and {Brighenti}, F. and {Brillet}, A. and {Brinkmann}, M. and {Brockill}, P. and {Brooks}, A.~F. and {Brooks}, J. and {Brown}, D.~D. and {Brunett}, S. and {Bruno}, G. and {Bruntz}, R. and {Buikema}, A. and {Bulik}, T. and {Bulten}, H.~J. and {Buonanno}, A. and {Buskulic}, D. and {Byer}, R.~L. and {Cabero}, M. and {Cadonati}, L. and {Caesar}, M. and {Cagnoli}, G. and {Cahillane}, C. and {Bustillo}, J. Calder{\'o}n and {Callaghan}, J.~D. and {Callister}, T.~A. and {Calloni}, E. and {Camp}, J.~B. and {Canepa}, M. and {Cannon}, K.~C. and {Cao}, H. and {Cao}, J. and {Carapella}, G. and {Carbognani}, F. and {Carney}, M.~F. and {Carpinelli}, M. and {Carullo}, G. and {Carver}, T.~L. and {Casanueva Diaz}, J. and {Casentini}, C. and {Caudill}, S. and {Cavagli{\`a}}, M. and {Cavalier}, F. and {Cavalieri}, R. and {Cella}, G. and {Cerd{\'a}-Dur{\'a}n}, P. and {Cesarini}, E. and {Chaibi}, W. and {Chakravarti}, K. and {Chan}, C. -L. and {Chan}, C. and {Chandra}, K. and {Chanial}, P. and {Chao}, S. and {Charlton}, P. and {Chase}, E.~A. and {Chassande-Mottin}, E. and {Chatterjee}, D. and {Chaturvedi}, M. and {Chen}, A. and {Chen}, H.~Y. and {Chen}, X. and {Chen}, Y. and {Cheng}, H. -P. and {Cheong}, C.~K. and {Chia}, H.~Y. and {Chiadini}, F. and {Chierici}, R. and {Chincarini}, A. and {Chiummo}, A. and {Cho}, G. and {Cho}, H.~S. and {Cho}, M. and {Choate}, S. and {Christensen}, N. and {Chu}, Q. and {Chua}, S. and {Chung}, K.~W. and {Chung}, S. and {Ciani}, G. and {Ciecielag}, P. and {Cie{\'s}lar}, M. and {Cifaldi}, M. and {Ciobanu}, A.~A. and {Ciolfi}, R. and {Cipriano}, F. and {Cirone}, A. and {Clara}, F. and {Clark}, E.~N. and {Clark}, J.~A. and {Clarke}, L. and {Clearwater}, P. and {Clesse}, S. and {Cleva}, F. and {Coccia}, E. and {Cohadon}, P. -F. and {Cohen}, D.~E. and {Colleoni}, M. and {Collette}, C.~G. and {Collins}, C. and {Colpi}, M. and {Constancio}, M., Jr. and {Conti}, L. and {Cooper}, S.~J. and {Corban}, P. and {Corbitt}, T.~R. and {Cordero-Carri{\'o}n}, I. and {Corezzi}, S. and {Corley}, K.~R. and {Cornish}, N. and {Corre}, D. and {Corsi}, A. and {Cortese}, S. and {Costa}, C.~A. and {Cotesta}, R. and {Coughlin}, M.~W. and {Coughlin}, S.~B. and {Coulon}, J. -P. and {Countryman}, S.~T. and {Couvares}, P. and {Covas}, P.~B. and {Coward}, D.~M. and {Cowart}, M.~J. and {Coyne}, D.~C. and {Coyne}, R. and {Creighton}, J.~D.~E. and {Creighton}, T.~D. and {Croquette}, M. and {Crowder}, S.~G. and {Cudell}, J.~R. and {Cullen}, T.~J. and {Cumming}, A. and {Cummings}, R. and {Cunningham}, L. and {Cuoco}, E. and {Curylo}, M. and {Dal Canton}, T. and {D{\'a}lya}, G. and {Dana}, A. and {DaneshgaranBajastani}, L.~M. and {D'Angelo}, B. and {Danilishin}, S.~L. and {D'Antonio}, S. and {Danzmann}, K. and {Darsow-Fromm}, C. and {Dasgupta}, A. and {Datrier}, L.~E.~H. and {Dattilo}, V. and {Dave}, I. and {Davier}, M. and {Davies}, G.~S. and {Davis}, D. and {Daw}, E.~J. and {Dean}, R. and {DeBra}, D. and {Deenadayalan}, M. and {Degallaix}, J. and {De Laurentis}, M. and {Del{\'e}glise}, S. and {Del Favero}, V. and {De Lillo}, N. and {Del Pozzo}, W. and {DeMarchi}, L.~M. and {De Matteis}, F. and {D'Emilio}, V. and {Demos}, N. and {Denker}, T. and {Dent}, T. and {Depasse}, A. and {De Pietri}, R. and {De Rosa}, R. and {De Rossi}, C. and {DeSalvo}, R. and {de Varona}, O. and {Dhurandhar}, S. and {D{\'\i}az}, M.~C. and {Diaz-Ortiz}, M., Jr. and {Didio}, N.~A. and {Dietrich}, T. and {Di Fiore}, L. and {DiFronzo}, C. and {Di Giorgio}, C. and {Di Giovanni}, F. and {Di Giovanni}, M. and {Di Girolamo}, T. and {Di Lieto}, A. and {Ding}, B. and {Di Pace}, S. and {Di Palma}, I. and {Di Renzo}, F. and {Divakarla}, A.~K. and {Dmitriev}, A. and {Doctor}, Z. and {D'Onofrio}, L. and {Donovan}, F. and {Dooley}, K.~L. and {Doravari}, S. and {Dorrington}, I. and {Downes}, T.~P. and {Drago}, M. and {Driggers}, J.~C. and {Du}, Z. and {Ducoin}, J. -G. and {Dupej}, P. and {Durante}, O. and {D'Urso}, D. and {Duverne}, P. -A. and {Dwyer}, S.~E. and {Easter}, P.~J. and {Eddolls}, G. and {Edelman}, B. and {Edo}, T.~B. and {Edy}, O. and {Effler}, A. and {Eichholz}, J. and {Eikenberry}, S.~S. and {Eisenmann}, M. and {Eisenstein}, R.~A. and {Ejlli}, A. and {Errico}, L. and {Essick}, R.~C. and {Estell{\'e}s}, H. and {Estevez}, D. and {Etienne}, Z.~B. and {Etzel}, T. and {Evans}, M. and {Evans}, T.~M. and {Ewing}, B.~E. and {Fafone}, V. and {Fair}, H. and {Fairhurst}, S. and {Fan}, X. and {Farah}, A.~M. and {Farinon}, S. and {Farr}, B. and {Farr}, W.~M. and {Fauchon-Jones}, E.~J. and {Favata}, M. and {Fays}, M. and {Fazio}, M. and {Feicht}, J. and {Fejer}, M.~M. and {Feng}, F. and {Fenyvesi}, E. and {Ferguson}, D.~L. and {Fernandez-Galiana}, A. and {Ferrante}, I. and {Ferreira}, T.~A. and {Fidecaro}, F. and {Figura}, P. and {Fiori}, I. and {Fiorucci}, D. and {Fishbach}, M. and {Fisher}, R.~P. and {Fishner}, J.~M. and {Fittipaldi}, R. and {Fitz-Axen}, M. and {Fiumara}, V. and {Flaminio}, R. and {Floden}, E. and {Flynn}, E. and {Fong}, H. and {Font}, J.~A. and {Forsyth}, P.~W.~F. and {Fournier}, J. -D. and {Frasca}, S. and {Frasconi}, F. and {Frei}, Z. and {Freise}, A. and {Frey}, R. and {Frey}, V. and {Fritschel}, P. and {Frolov}, V.~V. and {Fronz{\'e}}, G.~G. and {Fulda}, P. and {Fyffe}, M. and {Gabbard}, H.~A. and {Gadre}, B.~U. and {Gaebel}, S.~M. and {Gair}, J.~R. and {Gais}, J. and {Galaudage}, S. and {Gamba}, R. and {Ganapathy}, D. and {Ganguly}, A. and {Gaonkar}, S.~G. and {Garaventa}, B. and {Garc{\'\i}a-Quir{\'o}s}, C. and {Garufi}, F. and {Gateley}, B. and {Gaudio}, S. and {Gayathri}, V. and {Gemme}, G. and {Gennai}, A. and {George}, D. and {George}, J. and {Gergely}, L. and {Ghonge}, S. and {Ghosh}, Abhirup and {Ghosh}, Archisman and {Ghosh}, S. and {Giacomazzo}, B. and {Giacoppo}, L. and {Giaime}, J.~A. and {Giardina}, K.~D. and {Gibson}, D.~R. and {Gier}, C. and {Gill}, K. and {Giri}, P. and {Glanzer}, J. and {Gleckl}, A.~E. and {Godwin}, P. and {Goetz}, E. and {Goetz}, R. and {Gohlke}, N. and {Goncharov}, B. and {Gonz{\'a}lez}, G. and {Gopakumar}, A. and {Gossan}, S.~E. and {Gosselin}, M. and {Gouaty}, R. and {Grace}, B. and {Grado}, A. and {Granata}, M. and {Granata}, V. and {Grant}, A. and {Gras}, S. and {Grassia}, P. and {Gray}, C. and {Gray}, R. and {Greco}, G. and {Green}, A.~C. and {Green}, R. and {Gretarsson}, E.~M. and {Griggs}, H.~L. and {Grignani}, G. and {Grimaldi}, A. and {Grimes}, E. and {Grimm}, S.~J. and {Grote}, H. and {Grunewald}, S. and {Gruning}, P. and {Guerrero}, J.~G. and {Guidi}, G.~M. and {Guimaraes}, A.~R. and {Guix{\'e}}, G. and {Gulati}, H.~K. and {Guo}, Y. and {Gupta}, Anchal and {Gupta}, Anuradha and {Gupta}, P. and {Gustafson}, E.~K. and {Gustafson}, R. and {Guzman}, F. and {Haegel}, L. and {Halim}, O. and {Hall}, E.~D. and {Hamilton}, E.~Z. and {Hammond}, G. and {Haney}, M. and {Hanke}, M.~M. and {Hanks}, J. and {Hanna}, C. and {Hannam}, M.~D. and {Hannuksela}, O.~A. and {Hannuksela}, O. and {Hansen}, H. and {Hansen}, T.~J. and {Hanson}, J. and {Harder}, T. and {Hardwick}, T. and {Haris}, K. and {Harms}, J. and {Harry}, G.~M. and {Harry}, I.~W. and {Hartwig}, D. and {Hasskew}, R.~K. and {Haster}, C. -J. and {Haughian}, K. and {Hayes}, F.~J. and {Healy}, J. and {Heidmann}, A. and {Heintze}, M.~C. and {Heinze}, J. and {Heinzel}, J. and {Heitmann}, H. and {Hellman}, F. and {Hello}, P. and {Helmling-Cornell}, A.~F. and {Hemming}, G. and {Hendry}, M. and {Heng}, I.~S. and {Hennes}, E. and {Hennig}, J. and {Hennig}, M.~H. and {Vivanco}, F. Hernandez and {Heurs}, M. and {Hild}, S. and {Hill}, P. and {Hines}, A.~S. and {Hochheim}, S. and {Hofgard}, E. and {Hofman}, D. and {Hohmann}, J.~N. and {Holgado}, A.~M. and {Holland}, N.~A. and {Hollows}, I.~J. and {Holmes}, Z.~J. and {Holt}, K. and {Holz}, D.~E. and {Hopkins}, P. and {Horst}, C. and {Hough}, J. and {Howell}, E.~J. and {Hoy}, C.~G. and {Hoyland}, D. and {Huang}, Y. and {H{\"u}bner}, M.~T. and {Huddart}, A.~D. and {Huerta}, E.~A. and {Hughey}, B. and {Hui}, V. and {Husa}, S. and {Huttner}, S.~H. and {Hutzler}, B.~M. and {Huxford}, R. and {Huynh-Dinh}, T. and {Idzkowski}, B. and {Iess}, A. and {Imperato}, S. and {Inchauspe}, H. and {Ingram}, C. and {Intini}, G. and {Isi}, M. and {Iyer}, B.~R. and {JaberianHamedan}, V. and {Jacqmin}, T. and {Jadhav}, S.~J. and {Jadhav}, S.~P. and {James}, A.~L. and {Jani}, K. and {Janssens}, K. and {Janthalur}, N.~N. and {Jaranowski}, P. and {Jariwala}, D. and {Jaume}, R. and {Jenkins}, A.~C. and {Jeunon}, M. and {Jiang}, J. and {Johns}, G.~R. and {Jones}, A.~W. and {Jones}, D.~I. and {Jones}, J.~D. and {Jones}, P. and {Jones}, R. and {Jonker}, R.~J.~G. and {Ju}, L. and {Junker}, J. and {Kalaghatgi}, C.~V. and {Kalogera}, V. and {Kamai}, B. and {Kandhasamy}, S. and {Kang}, G. and {Kanner}, J.~B. and {Kapadia}, S.~J. and {Kapasi}, D.~P. and {Karathanasis}, C. and {Karki}, S. and {Kashyap}, R. and {Kasprzack}, M. and {Kastaun}, W. and {Katsanevas}, S. and {Katsavounidis}, E. and {Katzman}, W. and {Kawabe}, K. and {K{\'e}f{\'e}lian}, F. and {Keitel}, D. and {Key}, J.~S. and {Khadka}, S. and {Khalili}, F.~Y. and {Khan}, I. and {Khan}, S. and {Khazanov}, E.~A. and {Khetan}, N. and {Khursheed}, M. and {Kijbunchoo}, N. and {Kim}, C. and {Kim}, G.~J. and {Kim}, J.~C. and {Kim}, K. and {Kim}, W. and {Kim}, W.~S. and {Kim}, Y. -M. and {Kimball}, C. and {King}, P.~J. and {Kinley-Hanlon}, M. and {Kirchhoff}, R. and {Kissel}, J.~S. and {Kleybolte}, L. and {Klimenko}, S. and {Knowles}, T.~D. and {Knyazev}, E. and {Koch}, P. and {Koehlenbeck}, S.~M. and {Koekoek}, G. and {Koley}, S. and {Kolstein}, M. and {Komori}, K. and {Kondrashov}, V. and {Kontos}, A. and {Koper}, N. and {Korobko}, M. and {Korth}, W.~Z. and {Kovalam}, M. and {Kozak}, D.~B. and {Kr{\"a}mer}, C. and {Kringel}, V. and {Krishnendu}, N.~V. and {Kr{\'o}lak}, A. and {Kuehn}, G. and {Kumar}, A. and {Kumar}, P. and {Kumar}, Rahul and {Kumar}, Rakesh and {Kuns}, K. and {Kwang}, S. and {Lackey}, B.~D. and {Laghi}, D. and {Lalande}, E. and {Lam}, T.~L. and {Lamberts}, A. and {Landry}, M. and {Lane}, B.~B. and {Lang}, R.~N. and {Lange}, J. and {Lantz}, B. and {Lanza}, R.~K. and {Rosa}, I. La and {Lartaux-Vollard}, A. and {Lasky}, P.~D. and {Laxen}, M. and {Lazzarini}, A. and {Lazzaro}, C. and {Leaci}, P. and {Leavey}, S. and {Lecoeuche}, Y.~K. and {Lee}, H.~M. and {Lee}, H.~W. and {Lee}, J. and {Lee}, K. and {Lehmann}, J. and {Leon}, E. and {Leroy}, N. and {Letendre}, N. and {Levin}, Y. and {Li}, A. and {Li}, J. and {Li}, K.~J.~L. and {Li}, T.~G.~F. and {Li}, X. and {Linde}, F. and {Linker}, S.~D. and {Linley}, J.~N. and {Littenberg}, T.~B. and {Liu}, J. and {Liu}, X. and {Llorens-Monteagudo}, M. and {Lo}, R.~K.~L. and {Lockwood}, A. and {London}, L.~T. and {Longo}, A. and {Lorenzini}, M. and {Loriette}, V. and {Lormand}, M. and {Losurdo}, G. and {Lough}, J.~D. and {Lousto}, C.~O. and {Lovelace}, G. and {Lower}, M. and {L{\"u}ck}, H. and {Lumaca}, D. and {Lundgren}, A.~P. and {Ma}, Y. and {Macas}, R. and {MacInnis}, M. and {Macleod}, D.~M. and {MacMillan}, I.~A.~O. and {Macquet}, A. and {Maga{\~n}a Hernandez}, I. and {Maga{\~n}a-Sandoval}, F. and {Magazz{\`u}}, C. and {Magee}, R.~M. and {Majorana}, E. and {Maksimovic}, I. and {Maliakal}, S. and {Malik}, A. and {Man}, N. and {Mandic}, V. and {Mangano}, V. and {Mansell}, G.~L. and {Manske}, M. and {Mantovani}, M. and {Mapelli}, M. and {Marchesoni}, F. and {Marion}, F. and {M{\'a}rka}, S. and {M{\'a}rka}, Z. and {Markakis}, C. and {Markosyan}, A.~S. and {Markowitz}, A. and {Maros}, E. and {Marquina}, A. and {Marsat}, S. and {Martelli}, F. and {Martin}, I.~W. and {Martin}, R.~M. and {Martinez}, M. and {Martinez}, V. and {Martynov}, D.~V. and {Masalehdan}, H. and {Mason}, K. and {Massera}, E. and {Masserot}, A. and {Massinger}, T.~J. and {Masso-Reid}, M. and {Mastrogiovanni}, S. and {Matas}, A. and {Mateu-Lucena}, M. and {Matichard}, F. and {Matiushechkina}, M. and {Mavalvala}, N. and {Maynard}, E. and {McCann}, J.~J. and {McCarthy}, R. and {McClelland}, D.~E. and {McCormick}, S. and {McCuller}, L. and {McGuire}, S.~C. and {McIsaac}, C. and {McIver}, J. and {McManus}, D.~J. and {McRae}, T. and {McWilliams}, S.~T. and {Meacher}, D. and {Meadors}, G.~D. and {Mehmet}, M. and {Mehta}, A.~K. and {Melatos}, A. and {Melchor}, D.~A. and {Mendell}, G. and {Menendez-Vazquez}, A. and {Mercer}, R.~A. and {Mereni}, L. and {Merfeld}, K. and {Merilh}, E.~L. and {Merritt}, J.~D. and {Merzougui}, M. and {Meshkov}, S. and {Messenger}, C. and {Messick}, C. and {Metzdorff}, R. and {Meyers}, P.~M. and {Meylahn}, F. and {Mhaske}, A. and {Miani}, A. and {Miao}, H. and {Michaloliakos}, I. and {Michel}, C. and {Middleton}, H. and {Milano}, L. and {Miller}, A.~L. and {Millhouse}, M. and {Mills}, J.~C. and {Milotti}, E. and {Milovich-Goff}, M.~C. and {Minazzoli}, O. and {Minenkov}, Y. and {Mir}, Ll. M. and {Mishkin}, A. and {Mishra}, C. and {Mistry}, T. and {Mitra}, S. and {Mitrofanov}, V.~P. and {Mitselmakher}, G. and {Mittleman}, R. and {Mo}, G. and {Mogushi}, K. and {Mohapatra}, S.~R.~P. and {Mohite}, S.~R. and {Molina}, I. and {Molina-Ruiz}, M. and {Mondin}, M. and {Montani}, M. and {Moore}, C.~J. and {Moraru}, D. and {Morawski}, F. and {Moreno}, G. and {Morisaki}, S. and {Mours}, B. and {Mow-Lowry}, C.~M. and {Mozzon}, S. and {Muciaccia}, F. and {Mukherjee}, Arunava and {Mukherjee}, D. and {Mukherjee}, Soma and {Mukherjee}, Subroto and {Mukund}, N. and {Mullavey}, A. and {Munch}, J. and {Mu{\~n}iz}, E.~A. and {Murray}, P.~G. and {Nadji}, S.~L. and {Nagar}, A. and {Nardecchia}, I. and {Naticchioni}, L. and {Nayak}, R.~K. and {Neil}, B.~F. and {Neilson}, J. and {Nelemans}, G. and {Nelson}, T.~J.~N. and {Nery}, M. and {Neunzert}, A. and {Ng}, K.~Y. and {Ng}, S. and {Nguyen}, C. and {Nguyen}, P. and {Nguyen}, T. and {Nichols}, S.~A. and {Nissanke}, S. and {Nocera}, F. and {Noh}, M. and {North}, C. and {Nothard}, D. and {Nuttall}, L.~K. and {Oberling}, J. and {O'Brien}, B.~D. and {O'Dell}, J. and {Oganesyan}, G. and {Ogin}, G.~H. and {Oh}, J.~J. and {Oh}, S.~H. and {Ohme}, F. and {Ohta}, H. and {Okada}, M.~A. and {Olivetto}, C. and {Oppermann}, P. and {Oram}, R.~J. and {O'Reilly}, B. and {Ormiston}, R.~G. and {Ortega}, L.~F. and {O'Shaughnessy}, R. and {Ossokine}, S. and {Osthelder}, C. and {Ottaway}, D.~J. and {Overmier}, H. and {Owen}, B.~J. and {Pace}, A.~E. and {Pagano}, G. and {Page}, M.~A. and {Pagliaroli}, G. and {Pai}, A. and {Pai}, S.~A. and {Palamos}, J.~R. and {Palashov}, O. and {Palomba}, C. and {Pan}, H. and {Panda}, P.~K. and {Pang}, T.~H. and {Pankow}, C. and {Pannarale}, F. and {Pant}, B.~C. and {Paoletti}, F. and {Paoli}, A. and {Paolone}, A. and {Parker}, W. and {Pascucci}, D. and {Pasqualetti}, A. and {Passaquieti}, R. and {Passuello}, D. and {Patel}, M. and {Patricelli}, B. and {Payne}, E. and {Pechsiri}, T.~C. and {Pedraza}, M. and {Pegoraro}, M. and {Pele}, A. and {Penn}, S. and {Perego}, A. and {Perez}, C.~J. and {P{\'e}rigois}, C. and {Perreca}, A. and {Perri{\`e}s}, S. and {Petermann}, J. and {Petterson}, D. and {Pfeiffer}, H.~P. and {Pham}, K.~A. and {Phukon}, K.~S. and {Piccinni}, O.~J. and {Pichot}, M. and {Piendibene}, M. and {Piergiovanni}, F. and {Pierini}, L. and {Pierro}, V. and {Pillant}, G. and {Pilo}, F. and {Pinard}, L. and {Pinto}, I.~M. and {Piotrzkowski}, K. and {Pirello}, M. and {Pitkin}, M. and {Placidi}, E. and {Plastino}, W. and {Pluchar}, C. and {Poggiani}, R. and {Polini}, E. and {Pong}, D.~Y.~T. and {Ponrathnam}, S. and {Popolizio}, P. and {Porter}, E.~K. and {Poverman}, A. and {Powell}, J. and {Pracchia}, M. and {Prajapati}, A.~K. and {Prasai}, K. and {Prasanna}, R. and {Pratten}, G. and {Prestegard}, T. and {Principe}, M. and {Prodi}, G.~A. and {Prokhorov}, L. and {Prosposito}, P. and {Puecher}, A. and {Punturo}, M. and {Puosi}, F. and {Puppo}, P. and {P{\"u}rrer}, M. and {Qi}, H. and {Quetschke}, V. and {Quinonez}, P.~J. and {Quitzow-James}, R. and {Raab}, F.~J. and {Raaijmakers}, G. and {Radkins}, H. and {Radulesco}, N. and {Raffai}, P. and {Rafferty}, H. and {Rail}, S.~X. and {Raja}, S. and {Rajan}, C. and {Rajbhandari}, B. and {Rakhmanov}, M. and {Ramirez}, K.~E. and {Ramirez}, T.~D. and {Ramos-Buades}, A. and {Rana}, J. and {Rao}, K. and {Rapagnani}, P. and {Rapol}, U.~D. and {Ratto}, B. and {Raymond}, V. and {Razzano}, M. and {Read}, J. and {Reardon}, D.~J. and {Regimbau}, T. and {Rei}, L. and {Reid}, S. and {Reitze}, D.~H. and {Rettegno}, P. and {Ricci}, F. and {Richardson}, C.~J. and {Richardson}, J.~W. and {Richardson}, L. and {Ricker}, P.~M. and {Riemenschneider}, G. and {Riles}, K. and {Rizzo}, M. and {Robertson}, N.~A. and {Robinet}, F. and {Rocchi}, A. and {Rocha}, J.~A. and {Rodriguez}, S. and {Rodriguez-Soto}, R.~D. and {Rolland}, L. and {Rollins}, J.~G. and {Roma}, V.~J. and {Romanelli}, M. and {Romano}, R. and {Romel}, C.~L. and {Romero}, A. and {Romero-Shaw}, I.~M. and {Romie}, J.~H. and {Ronchini}, S. and {Rose}, C.~A. and {Rose}, D. and {Rose}, K. and {Rosi{\'n}ska}, D. and {Rosofsky}, S.~G. and {Ross}, M.~P. and {Rowan}, S. and {Rowlinson}, S.~J. and {Roy}, Santosh and {Roy}, Soumen and {Ruggi}, P. and {Ryan}, K. and {Sachdev}, S. and {Sadecki}, T. and {Sadiq}, J. and {Sakellariadou}, M. and {Salafia}, O.~S. and {Salconi}, L. and {Saleem}, M. and {Samajdar}, A. and {Sanchez}, E.~J. and {Sanchez}, J.~H. and {Sanchez}, L.~E. and {Sanchis-Gual}, N. and {Sanders}, J.~R. and {Santiago}, K.~A. and {Santos}, E. and {Saravanan}, T.~R. and {Sarin}, N. and {Sassolas}, B. and {Sauter}, O. and {Savage}, R.~L. and {Savant}, V. and {Sawant}, D. and {Sayah}, S. and {Schaetzl}, D. and {Schale}, P. and {Scheel}, M. and {Scheuer}, J. and {Schindler-Tyka}, A. and {Schmidt}, P. and {Schnabel}, R. and {Schofield}, R.~M.~S. and {Sch{\"o}nbeck}, A. and {Schreiber}, E. and {Schulte}, B.~W. and {Schutz}, B.~F. and {Schwarm}, O. and {Schwartz}, E. and {Scott}, J. and {Scott}, S.~M. and {Seglar-Arroyo}, M. and {Seidel}, E. and {Sellers}, D. and {Sengupta}, A.~S. and {Sennett}, N. and {Sentenac}, D. and {Sequino}, V. and {Sergeev}, A. and {Setyawati}, Y. and {Shaffer}, T. and {Shahriar}, M.~S. and {Sharifi}, S. and {Sharma}, A. and {Sharma}, P. and {Shawhan}, P. and {Shen}, H. and {Shikauchi}, M. and {Shink}, R. and {Shoemaker}, D.~H. and {Shoemaker}, D.~M. and {Shukla}, K. and {ShyamSundar}, S. and {Sieniawska}, M. and {Sigg}, D. and {Singer}, L.~P. and {Singh}, D. and {Singh}, N. and {Singha}, A. and {Singhal}, A. and {Sintes}, A.~M. and {Sipala}, V. and {Skliris}, V. and {Slagmolen}, B.~J.~J. and {Slaven-Blair}, T.~J. and {Smetana}, J. and {Smith}, J.~R. and {Smith}, R.~J.~E. and {Somala}, S.~N. and {Son}, E.~J. and {Soni}, S. and {Sorazu}, B. and {Sordini}, V. and {Sorrentino}, F. and {Sorrentino}, N. and {Soulard}, R. and {Souradeep}, T. and {Sowell}, E. and {Spencer}, A.~P. and {Spera}, M. and {Srivastava}, A.~K. and {Srivastava}, V. and {Staats}, K. and {Stachie}, C. and {Steer}, D.~A. and {Steinke}, M. and {Steinlechner}, J. and {Steinlechner}, S. and {Steinmeyer}, D. and {Stolle-McAllister}, G. and {Stops}, D.~J. and {Stover}, M. and {Strain}, K.~A. and {Stratta}, G. and {Strunk}, A. and {Sturani}, R. and {Stuver}, A.~L. and {S{\"u}dbeck}, J. and {Sudhagar}, S. and {Sudhir}, V. and {Summerscales}, T.~Z. and {Sun}, H. and {Sun}, L. and {Sunil}, S. and {Sur}, A. and {Suresh}, J. and {Sutton}, P.~J. and {Swinkels}, B.~L. and {Szczepa{\'n}czyk}, M.~J. and {Tacca}, M. and {Tait}, S.~C. and {Talbot}, C. and {Tanasijczuk}, A.~J. and {Tanner}, D.~B. and {Tao}, D. and {Tapia}, A. and {San Martin}, E.~N. Tapia and {Tasson}, J.~D. and {Taylor}, R. and {Tenorio}, R. and {Terkowski}, L. and {Thirugnanasambandam}, M.~P. and {Thomas}, M. and {Thomas}, P. and {Thompson}, J.~E. and {Thondapu}, S.~R. and {Thorne}, K.~A. and {Thrane}, E. and {Tiwari}, Shubhanshu and {Tiwari}, Srishti and {Tiwari}, V. and {Toland}, K. and {Tolley}, A.~E. and {Tonelli}, M. and {Tornasi}, Z. and {Torres-Forn{\'e}}, A. and {Torrie}, C.~I. and {e Melo}, I. Tosta and {T{\"o}yr{\"a}}, D. and {Tran}, A.~T. and {Trapananti}, A. and {Travasso}, F. and {Traylor}, G. and {Tringali}, M.~C. and {Tripathee}, A. and {Trovato}, A. and {Trudeau}, R.~J. and {Tsai}, D.~S. and {Tsang}, K.~W. and {Tse}, M. and {Tso}, R. and {Tsukada}, L. and {Tsuna}, D. and {Tsutsui}, T. and {Turconi}, M. and {Ubhi}, A.~S. and {Udall}, R.~P. and {Ueno}, K. and {Ugolini}, D. and {Unnikrishnan}, C.~S. and {Urban}, A.~L. and {Usman}, S.~A. and {Utina}, A.~C. and {Vahlbruch}, H. and {Vajente}, G. and {Vajpeyi}, A. and {Valdes}, G. and {Valentini}, M. and {Valsan}, V. and {van Bakel}, N. and {van Beuzekom}, M. and {van den Brand}, J.~F.~J. and {Van Den Broeck}, C. and {Vander-Hyde}, D.~C. and {van der Schaaf}, L. and {van Heijningen}, J.~V. and {Vardaro}, M. and {Vargas}, A.~F. and {Varma}, V. and {Vass}, S. and {Vas{\'u}th}, M. and {Vecchio}, A. and {Vedovato}, G. and {Veitch}, J. and {Veitch}, P.~J. and {Venkateswara}, K. and {Venneberg}, J. and {Venugopalan}, G. and {Verkindt}, D. and {Verma}, Y. and {Veske}, D. and {Vetrano}, F. and {Vicer{\'e}}, A. and {Viets}, A.~D. and {Villa-Ortega}, V. and {Vinet}, J. -Y. and {Vitale}, S. and {Vo}, T. and {Vocca}, H. and {Vorvick}, C. and {Vyatchanin}, S.~P. and {Wade}, A.~R. and {Wade}, L.~E. and {Wade}, M. and {Walet}, R.~C. and {Walker}, M. and {Wallace}, G.~S. and {Wallace}, L. and {Walsh}, S. and {Wang}, J.~Z. and {Wang}, S. and {Wang}, W.~H. and {Wang}, Y.~F. and {Ward}, R.~L. and {Warner}, J. and {Was}, M. and {Washington}, N.~Y. and {Watchi}, J. and {Weaver}, B. and {Wei}, L. and {Weinert}, M. and {Weinstein}, A.~J. and {Weiss}, R. and {Wellmann}, F. and {Wen}, L. and {We{\ss}els}, P. and {Westhouse}, J.~W. and {Wette}, K. and {Whelan}, J.~T. and {White}, D.~D. and {White}, L.~V. and {Whiting}, B.~F. and {Whittle}, C. and {Wilken}, D.~M. and {Williams}, D. and {Williams}, M.~J. and {Williamson}, A.~R. and {Willis}, J.~L. and {Willke}, B. and {Wilson}, D.~J. and {Wimmer}, M.~H. and {Winkler}, W. and {Wipf}, C.~C. and {Woan}, G. and {Woehler}, J. and {Wofford}, J.~K. and {Wong}, I.~C.~F. and {Wrangel}, J. and {Wright}, J.~L. and {Wu}, D.~S. and {Wysocki}, D.~M. and {Xiao}, L. and {Yamamoto}, H. and {Yang}, L. and {Yang}, Y. and {Yang}, Z. and {Yap}, M.~J. and {Yeeles}, D.~W. and {Yoon}, A. and {Yu}, Hang and {Yu}, Haocun and {Yuen}, S.~H.~R. and {Zadro{\.z}ny}, A. and {Zanolin}, M. and {Zelenova}, T. and {Zendri}, J. -P. and {Zevin}, M. and {Zhang}, J. and {Zhang}, L. and {Zhang}, R. and {Zhang}, T. and {Zhao}, C. and {Zhao}, G. and {Zhou}, M. and {Zhou}, Z. and {Zhu}, X.~J. and {Zucker}, M.~E. and {Zweizig}, J. and {LIGO Scientific Collaboration} and {Virgo Collaboration} and {Keith}, M.~J. and {Lyne}, A.~G. and {Palfreyman}, J. and {Shaw}, B. and {Stappers}, B.~W. and {Weltevrede}, P.},
        title = "{Gravitational-wave Constraints on the Equatorial Ellipticity of Millisecond Pulsars}",
      journal = {\apjl},
     keywords = {Gravitational waves, Neutron stars, Pulsars, Gravitational wave sources, 678, 1108, 1306, 677, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2020,
        month = oct,
       volume = {902},
       number = {1},
          eid = {L21},
        pages = {L21},
          doi = {10.3847/2041-8213/abb655},
archivePrefix = {arXiv},
       eprint = {2007.14251},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...902L..21A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...863L..40W,
       author = {{Woan}, G. and {Pitkin}, M.~D. and {Haskell}, B. and {Jones}, D.~I. and {Lasky}, P.~D.},
        title = "{Evidence for a Minimum Ellipticity in Millisecond Pulsars}",
      journal = {\apjl},
     keywords = {gravitational waves, pulsars: general, stars: magnetic field, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2018,
        month = aug,
       volume = {863},
       number = {2},
          eid = {L40},
        pages = {L40},
          doi = {10.3847/2041-8213/aad86a},
archivePrefix = {arXiv},
       eprint = {1806.02822},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...863L..40W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983ApJ...272..286G,
       author = {{Gudmundsson}, E.~H. and {Pethick}, C.~J. and {Epstein}, R.~I.},
        title = "{Structure of neutron star envelopes}",
      journal = {\apj},
     keywords = {Neutron Stars, Stellar Envelopes, Stellar Structure, Density (Mass/Volume), Gravitation, Opacity, Stellar Luminosity, Stellar Temperature, Surface Temperature, Astrophysics},
         year = 1983,
        month = sep,
       volume = {272},
        pages = {286-300},
          doi = {10.1086/161292},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983ApJ...272..286G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015SSRv..191..239P,
       author = {{Potekhin}, Alexander Y. and {Pons}, Jos{\'e} A. and {Page}, Dany},
        title = "{Neutron Stars{\textemdash}Cooling and Transport}",
      journal = {\ssr},
     keywords = {Neutron stars, Magnetic fields, Dense matter, Thermal emission, Heat transport, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = oct,
       volume = {191},
       number = {1-4},
        pages = {239-291},
          doi = {10.1007/s11214-015-0180-9},
archivePrefix = {arXiv},
       eprint = {1507.06186},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015SSRv..191..239P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...457..844L,
       author = {{Link}, Bennett and {Epstein}, Richard I.},
        title = "{Thermally Driven Neutron Star Glitches}",
      journal = {\apj},
     keywords = {DENSE MATTER, STARS: EVOLUTION, STARS: INTERIORS, STARS: NEUTRON, Astrophysics},
         year = 1996,
        month = feb,
       volume = {457},
        pages = {844},
          doi = {10.1086/176779},
archivePrefix = {arXiv},
       eprint = {astro-ph/9508021},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...457..844L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.333..613L,
       author = {{Larson}, Michelle B. and {Link}, Bennett},
        title = "{Simulations of glitches in isolated pulsars}",
      journal = {\mnras},
     keywords = {dense matter, stars: evolution, stars: interiors, stars: neutron, stars: rotation, Astrophysics},
         year = 2002,
        month = jul,
       volume = {333},
       number = {3},
        pages = {613-622},
          doi = {10.1046/j.1365-8711.2002.05439.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0105461},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.333..613L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


